Near Optimal Adversarial Attacks on Stochastic Bandits and Defenses with Smoothed Responses

I study adversarial attacks against stochastic bandit algorithms. At each round, the learner chooses an arm, and a stochastic reward is generated. The adversary strategically adds corruption to the reward, and the learner is only able to observe the corrupted reward at each round. Two sets of results are presented in this paper. The first set studies the optimal attack strategies for the adversary. The adversary has a target arm he wishes to promote, and his goal is to manipulate the learner into choosing this target arm $T - o(T)$ times. I design attack strategies against UCB and Thompson Sampling that only spend $\widehat{O}(\sqrt{\log T})$ cost. Matching lower bounds are presented, and the vulnerability of UCB, Thompson sampling, and $\varepsilon$-greedy are exactly characterized. The second set studies how the learner can defend against the adversary. Inspired by literature on smoothed analysis and behavioral economics, I present two simple algorithms that achieve a competitive ratio arbitrarily close to 1.

==> color-edits.tex <==
\ProvidesPackage{color-edits}

\def\@SuppressEdits{no}
\DeclareOption{suppress}{%
\def\@SuppressEdits{yes}
}

\def\@ShowDeletions{no}
\DeclareOption{showdeletions}{\def\@ShowDeletions{yes}}

\ProcessOptions

% Provides useful macros for making recent edits by different authors
% visible with colors in a jointly edited LaTeX document.
% Different authors are added with \addauthor{AUTH}{color}
% (the only exported command provided by this package).
% Invocation of \addauthor generates four new commands
% (where AUTH should be replaced by the supplied name of the author,
% e.g., initials, or whatever else is used):
% 1. \AUTHedit{text}: displayes the 'text' in the color assigned to the
% author.
% 2. \AUTHcomment{text}: generates '[AUTH: text]' in the color
% assigned, i.e., annotates the text as a comment written by the
% author.
% 3. \AUTHmargincomment{text}: generates a marker in the author's
% color at the given spot, and writes the text in the color in the
% margin. 
% 4. \AUTHdelete{text}: per default, displays a marker in the author's
% color at the given spot, and marks in the margin that the author
% deleted something in this place. (This allows co-authors to check
% what was deleted.)
%
% As an example, \addauthor{dk}{blue} generates the commands
% \dkedit{}, \dkcomment{}, \dkmargincomment{}, \dkdelete{}, all of
% which display material in blue.
%
% The package allows two options:
% 1. 'suppress' suppresses all comments and deletion markers, and
% removes the coloring from text in \AUTHedit{}. Thus, it essentially
% displays the text as it would be once all comments are explicitly
% removed (though there may be small spacing issues, so they should
% still be explicitly removed eventually).
% 2. 'showdeletions' replaces the semantics of the \AUTHdelete{text}
% command, so that instead the text is still displayed, but struck out
% (and in the color of the coresponding author). This allows
% co-authors to see more easily what has been deleted, without having
% to check the source code.

\usepackage{ifthen}
\usepackage{color}
\usepackage{marginnote}
\usepackage[normalem]{ulem}

\newcommand{\@edit}[2]{%
\ifthenelse{\equal{\@SuppressEdits}{yes}}{#2}{\textcolor{#1}{#2}}%
}

\newcommand{\@comment}[2]{%
\ifthenelse{\equal{\@SuppressEdits}{yes}}{}{\textcolor{#1}{#2}}%
}

\newcommand{\@margincomment}[2]{%
\ifthenelse{\equal{\@SuppressEdits}{yes}}{}{%
\marginnote{\scriptsize\textcolor{#1}{#2}}%
}}

\newcommand{\@delete}[3]{%
\ifthenelse{\equal{\@SuppressEdits}{yes}}{}{%
\ifthenelse{\equal{\@ShowDeletions}{yes}}{%
\textcolor{#1}{\ifmmode\text{\sout{\ensuremath{#2}}}\else\sout{#2}\fi}}{%
\textcolor{#1}{\ensuremath{[\bullet]}}%
\marginnote{\scriptsize\textcolor{#1}{#3 deleted here}}}}%
}

\newcommand{\addauthor}[2]{%
\expandafter\def\csname #1edit\endcsname ##1{\@edit{#2}{##1}}
\expandafter\def\csname #1comment\endcsname ##1{\@comment{#2}{[#1: ##1]}}
\expandafter\def\csname #1margincomment\endcsname ##1{\@margincomment{#2}{[#1: ##1]}}
\expandafter\def\csname #1delete\endcsname ##1{\@delete{#2}{##1}{#1}}
}

==> notations_old.tex <==
%\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
%\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand{\Q}[1]{\item {[{\em #1 pts\/}]}\ }
\newcommand{\fighere}[2]{\begin{figure}[h]\begin{center}%
  \includegraphics[scale=#2]{#1.pdf}\end{center}%
  \end{figure}\vspace{-\bigskipamount}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\Ex}{\mathbb{E}}
\newcommand{\Var}{\mathbb{V}}
\newcommand{\eps}{\varepsilon}
\newcommand{\OO}{\widetilde{O}}
\newcommand{\down}[1]{\left\lfloor #1\right\rfloor}
\newcommand{\up}[1]{\left\lceil #1\right\rceil}
\newcommand{\IGNORE}[1]{}
\newcommand{\hatO}{\widehat{O}}

\renewcommand{\ip}[2]{\langle #1, #2\rangle}
\newcommand{\ind}[1]{\mathbbm{1}\{#1\}}

\newcommand{\RegNN}{\mathrm{Reg}_\texttt{NN}}
\newcommand{\RegCB}{\mathrm{Reg}_\texttt{CB}}
\newcommand{\Ball}{\mathcal{B}}
\newcommand{\hatmu}{\hat{\mu}}


\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}
\newtheorem{claim}{Claim}
\newtheorem{example}{Example}




==> otherNotes/competitiveRatio.tex <==
\section{Optimizing the Competitive Ratio}
We will assume rewards are bounded in this section $[0,1]$. 

It is not hard to see there does not exist algorithm that achieve good performance against strong adversary. So I will turn attention to optimizing the competitive ratio. 


\begin{definition}
\[
\Ex[\REW] \ge \frac{\OPT}{\beta}
\]
\end{definition}

It will not be hard to obtain $\log T$ competitive ratio in expectation. Maintain $\log T$ copies of algorithm, each robust to corruption level $C = 2^h$. 

With probability $1/\log T$, the correct layer is chosen, and
\[
\Ex[\REW] \ge \OPT - o(T)
\]

Our goal will be to convert this to high probability. 

Give a lower bound first. 


==> otherNotes/detection.tex <==
\section{Defense with a detection technology}
The previous results seem too pessimistic, and in part, this is due to the strong power of the adversary. Indeed, previous works have observed any bandit algorithm achieving $O(\log T)$ regret, the adversary can spend only $O(\log T)$ attack cost and completely hijack the algorithm. In this section, I study a model where the learner is equipped with more power. Specifically, he is equipped with a corruption detection system. At each round, the detection system returns a noisy binary signal. A signal of 0 means that no corruption has been detected, and a signal of 1 means that corruption has been detected. 
\begin{assumption}
When the adversary injects corruption $\alpha$, $\cS$ returns 1 with probability $p(\abs{\alpha})$. Moreover, $p$ is strictly increasing. 
\end{assumption}

I now design low-regret algorithms for the learner. \szcomment{Idea 1: use ratio of 0-signal / 1 signal. Idea 2: use ratio of $c_t / p(c_t)$}

\begin{algorithm}

\end{algorithm}

At time $t$, consider queries on some arm $a$. Let $S_{a}^0$ denote the observed reward on rounds in which the detection signal is $s = 0$, let $S_{a}^1$ be rounds in which $s = 1$. 

\begin{definition}
Define the growth function $g(\beta)$ as the function satisfying
\[
p(x) > \frac{x}{g(x)} 
\]
In other words, $p(x)$ lies above the function with slope $1/g(beta)$ when $x > \beta$. 
\end{definition}

\begin{lemma}
\[
\Ex[D_t] = \sum_t p(\alpha_t)
\]
\end{lemma}

\begin{lemma}
\[
\frac{\sum \alpha_t}{n} < xxx
\]
\end{lemma}

\begin{proof}
\begin{align*}
\frac{\sum \alpha_t}{n} &= \sum \frac{\alpha_t}{p(c_t)} \frac{p(c_t)}{n} \\
&\le \inf_\beta \frac{\sum (\alpha_t|\alpha_t < \beta) + (\alpha_t|\alpha_t >\beta) }{n}\\
&\le \inf_\beta \beta + \frac{\sum\alpha_t >\beta}{n} \\
&\le \inf_\beta \beta + \sum\frac{\alpha_t}{p(\alpha_t)} \frac{p(\alpha_t)}{t} \ind{\alpha_t > \beta} \\
&\le \inf_\beta \beta + g(\beta) \frac{\sum p(\alpha_t)} {t} \\\
&\lesssim \inf_\beta \beta + g(\beta) \frac{D_t}{t}
\end{align*}
\end{proof}

\begin{lemma}
\[
{\mu}_a \lesssim \hat{\mu}_a + \inf_\beta \beta + g(\beta) \frac{D_{a,t}}{N_{a,t}} + \sqrt{ \frac{\log T}{N_{a,t}} }
\]
\end{lemma}


Fix a corruption level $\beta$. Fix round $t$. Let $N_{>\beta}^0$ be rounds in which $s = 0$, let $N_{>\beta}^1$ be rounds in which $s = 1$. Let $N_{>\beta}$ be the total rounds in which corruption is $>\beta$. 
\begin{lemma}
With high probability: 
\[
N_{>\beta}^0 <\approx (1 - p(\beta)) N_{>\beta}. 
\]
\end{lemma}

Construct C-UCB as follows. 
\begin{lemma}
Fix $\beta$, round $t$ and arm $a$. Let $N_1(t)$ be number detected rounds. Then $\hatmu_{a} < xxx$
\end{lemma}
\begin{proof}
By previous lemma, $N_{>\beta}^0 \lesssim (1-p(\beta)) N^1$. 

Let's focus on the empirical mean of $\hat{\mu}^0_a$ in $S^{0}$. 
\begin{align*}
\hat{\mu}^0_a &= \frac{\sum r^0_t}{N} < \frac{\sum r_t + N_{>\beta}^0}{N} + \beta \\
&< \hat{\mu}_a + \frac{N_{>\beta}^0}{N} + \beta
\end{align*}



\end{proof}


==> otherNotes/detection_notes.tex <==
\section{Defense using Probalistic Detection - notes}

Suppose the arms give bernoulli rewards. As usual, the adversary has some target arm he wishes to promote. However, now we assume the learner has a defense technology: she can detect corruptions probabilistically. Let there be $K$ arms, each generating Bernoulli rewards with mean $\mu_a$. At each round, the adversary can decide the corrupt the reward (flip from 0 to 1 or from 1 to 0). If the adversary corrupts the reward, the learner detects a signal with probability $p_H$. If the adversary does not corrupt the reward, the learner detects a signal with probability $p_L$. 

We first show naive-UCB by simplying ignoring corrupted rounds does not work. The adversary employs the strategy where he always lowers non-target arms to $0$ whenever pulled. With probability $p_H$ he gets detected, but he does not care. 

Now we consider the following algorithm. The learner computes a modified UCB index. Or he ensures the number of non-detected rounds is more than the number of detected rounds by some threshold. Maybe better to use Thompson Sampling or Bayesian updates. 
 
\subsection{Robust UCB with probablistic detection}
Naive UCB compute index as $...$. At each round, can we have unbiased estimate of reward? No, so have to work with biased estimates. 

\begin{algorithm}
\caption{Some algorithm}
\label{algo:UCBDefense}
\begin{algorithmic}
\STATE For each arm $a$, maintain two sets $S^{nd}_a$ and $S^d_a$, the first set records data with no reported detection and the second set records data with reported detections
\FOR {$t = 1, \dots, T$}
    \STATE For each arm $a$, compute the modified UCB index as
    \STATE Alternative: pull this arm $a$ until the size of $S^{nd}$ and $ S^d$ satisfy certain condition. This needs $S^{nd} > \omega(S^d)$ and that $S^{nd}$ is big enough. 
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsubsection{Sketch Notes}
Consider all rounds that arm $a$ is pulled. Some of them will be corrupted, others are not. Let $c_t$ denote the indicator variable that the adversary corrupted the signal in round $t$, let $d_t$ denote the random variable that a detection was reported to the learner. $d_t$ takes value $\set{0,1}$. 

Let $H_t$ denote the history that includes all data up to time $t$. 

Then
\begin{lemma}
\[
\Ex[D_t | c_t, H_{t-1}] = p_H \text{ or } p_L
\]
\end{lemma}

\begin{lemma}
Fix time $t$ and focus on the rounds in which arm $a$ is pulled. Let $C_t$ be the number of corrupted rounds. Let $D_t$ be the number of detected rounds. Then $\Ex[D_t] = C_t \cdot p_H$. 
\end{lemma}

Moving on to bounded rewards... Rewards are bounded in $[0,1]$. Each arm gives a reward centered at mean $\mu_a$. Corruption of $\alpha$ leads to detection probability of $f(\alpha)$. Suppose we want a $\delta$-accurate estimate of $\mu_a$. How do we do this? Query this arm so that the size of $S^{nd}$ and $S^d$ are large. Let $\rho(\delta_0) = p(\delta_0) / (1-p(\delta_0))$ be the likelihood function. 

\begin{lemma}
If $S^{nd} \dots $, then we have $\delta_0$ estimate for the mean. 
\end{lemma}

\begin{proof}
Let $N^{nd}_{>\delta_0}$ be the number of non-detected rounds when corruption is at least $\delta_0$. Let $N^{d}_{>\delta_0}$ be the number of detected rounds when corruption is at least $\delta_0$. Let $N^{nd}_{<\delta_0}$ and $N^d_{<\delta_0}$ be as defined similarly. Then
\[
N^d_{>\delta_0} < N^d. 
\]
With high probability:
\[
N^{nd}_{<\delta_0} < O(\rho) \cdot N^D_{>\delta_0}
\]
So a large fraction from the non-detected pool come from corruption less than $< \delta_0$. 

Consider the following statistic: $\bar{Y} := $ the sample mean of all observations less the lowest $O(\rho) N^d$ order statistics. 

We would like some concentration results on $\bar{Y}$. Let $\bar{Y^0}$ be the pre-attack rewards for the top order statistics. Let $\bar{X^0}$ be the pre-attack rewards in the set $S^{nd}$. Then
\[
\bar{Y_0} \frac{N}{N^{nd}} < \bar{X_0} < \frac {\bar{Y_0} N + N^{nd} - N} {N^{nd}}
\]
Equivalently:
\[
\bar{Y_0} > \frac{\bar{X_0} N^{nd} + N - N^{nd} }{N} 
\]
Ensure $\frac{N^{nd}}{N_{<\delta}} < 1 + \delta_1$ for now. Then
\[
\bar{Y_0} > \frac{\bar{X_0} N^{nd} + N_{<\delta} - N^{nd} } {N_{\delta}} 
\]

Then the following can be bounded! 
\begin{align*}
\Pr[\bar{Y} > \mu - t] &< \Pr[\bar{Y^0} > \mu - t + \delta_0] \\
&< \Pr[ \bar{X_0}\frac{N^{nd}}{N} - \frac{N^{nd} - N}{N} \ge \mu + 2\delta_0] \\
&= \Pr[ \bar{X_0} \ge \mu - t + 3\delta_0] \\
&< \Pr[ \dots  ]
\end{align*}

The first line is because attacks are bounded above by $\delta_0$. 

So we can indeed have accurate estimate on $\bar{Y}$. 

\end{proof}

\subsection{Corrected-ETC}
I introduce the Corrected-ETC (CETC) algorithm. Assume the minimum gap $\Delta_\min$ is known. Now we find $\Delta_\min / 2$ estimates for the unknown mean. 

\subsection{Analysis}
\begin{lemma}
Let $X = \set{X_1, \dots, X_n}$ be independent samples from a distribution supported on $[0,1]$. Let $Y = \set{Y_1, \dots, Y_n}$ satisfy at least $m$ are $\delta$ close to the original value. Let $\wbar{Y_\top}$ be the mean of the top $m$ order statistics. Then 
\[
\Pr[\mu > \wbar{Y_\top} + \eta] < \dots
\]
and
\[
\Pr[\mu < \wbar{Y_\low} - \eta] < \dots
\]
\end{lemma}
\begin{proof}
Let $\wbar{X}$ denote the sample mean. Then we have
\[
\frac{\wbar{Y_\low} m} {n} - \delta \le \wbar{X} \le \frac{ \wbar{Y_\top} m + n - m}{n} + \delta
\]
Since by standard Hoeffding:
\[
\Pr[\mu > \wbar{X} + \eta] < xxx
\]
and
\[
\Pr[\mu < \wbar{X} - \eta] < xxx
\]
We must have
\[
\Pr[\mu > \wbar{Y_\top}\frac{m}{n} + \frac{n-m}{n} + \eta] < xxx
\]
and
\[
\Pr[\mu < \wbar{Y_\low} \frac{m}{n} - \eta] < xxx
\]
In other words, with probability at least xxx:
\[
\wbar{Y_\low} \frac{m}{n} - \eta < \mu < \wbar{Y_\top}\frac{m}{n} + \frac{n-m}{n} + \eta
\]
So we will need $\frac{n-m}{n} = O(\eta)$ and $n = \Omega(\log T)$. 
\end{proof}

\subsection{Robust Thompson Sampling}
Naive Thompson Sampling sample from $\Beta(1+\alpha, 1+\beta)$. We need to adjust this. Suppose we have some prior on the mean $\mu_a$. We now observe possibly corrupted reward $r_t$ and detection signal $d_t$. How can we update the posterior?

==> otherNotes/robustAlgo.tex <==
\section{Thompson Sampling is Robust? }
\subsection{Thomspon sampling papers}
Analysis of thompson sampling for the multi-armed bandit problem

Further optimal regret bounds for Thompson sampling.

Near-optimal regret bounds for thompson sampling

Thompson sampling: An asymptotically
optimal finite-time analysis

Thompson sampling for 1-dimensional
exponential family bandits. 

\subsection{Notes}

Consider the Thompson sampling algorithm. Where at each round, a random variable is sampled from
\[
\cN(\hat{\mu}_a, \frac{1}{N_a(t)}). 
\]

The sample probability of a seemingly inferior arm can be lower bounded by:
\[
\cN(\hat{\mu}_a - \hat{\mu}^*, \frac{1}{N_a(t)}) \ge \Omega ( \exp( - N_a(t) ) )
\]
\szcomment{Also depend on gap. }

The probability that arm $a$ is pulled should be set as:
\[
\Omega ( \exp( - N_a(t) ) ). 
\]

So the expected number of pulls until the next pull is $ \exp(N_a(t)) $. 

Suppose the two arms give rewards centered at $\mu_1$ and $\mu_2$ and $\mu_1 < \mu_2$. So the adversary will attack arm 2. 

Consider the round in which arm 2 has been pulled for exactly $N$ times. 

Let $a$ be some suboptimal arm. 
If no corruption, suboptimal arm $\log T / \Delta_a$ times. 

If corruption, suboptimal arm total $C_a / \Delta_a$ times. 

Show correct arm identified after $C + K\log C$ rounds. 

Consider only two arms. 


==> otherNotes/table_old.tex <==
\begin{tabular}{l|l|lll}
\hline
Approach & $\sigma$   & $\mu = 0.1$ & $\mu = 1$ & $ \mu = 2$ \\ \hline
\cite{jun2018adversarial}      & $\sigma = 0.1$ & 23.6        & 129.4     & 247.3      \\ \hline
This work      & $\sigma$ = 0.1  & 1.3         & 2.4       & 3.6        \\ \hline
This work        & $\sigma$ = 1  & 14.5        & 15.9      & 16.8       \\ \hline
This work        & $\sigma$ = 2  & 30.3        & 30.7      & 31.0       \\ \hline
\end{tabular}

\begin{table}
\parbox{.45\linewidth}{
\centering
\begin{tabular}{l|l|lll}
\hline
Approach & $\sigma$   & $\mu = 0.1$ & $\mu = 1$ & $ \mu = 2$ \\ \hline
\cite{jun2018adversarial}      &  0.1 & 23.6        & 129.4     & 247.3      \\ \hline
This work      &  0.1  & 1.3         & 2.4       & 3.6        \\ \hline
This work        &  1  & 14.5        & 15.9      & 16.8       \\ \hline
This work        &  2  & 30.3        & 30.7      & 31.0       \\ \hline
\end{tabular}
\caption{Attack cost on UCB}
\label{table:attackUCB}
}
\hfill
\parbox{.45\linewidth}{
\centering
\begin{tabular}{l|lll}
\hline
$\sigma$ & $\mu = 0.1$ & $\mu = 1$ & $ \mu = 2$ \\ \hline
0.1      & 13.0        & 13.9      & 15.0       \\ \hline
1        & 19.0        & 19.7      & 20.6       \\ \hline
2        & 23.8        & 25.0      & 26.7       \\ \hline
\end{tabular}
\caption{Attack cost on Thompson sampling}
\label{table:attackTS}
}
\end{table}

==> sections/checklist.tex <==
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%

% %%% END INSTRUCTIONS %%%


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   %\item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [No]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Not Applicable]
    \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
    \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not Applicable]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Not Applicable]
   \item The license information of the assets, if applicable. [Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}
